Dichotomy for symmetric Boolean PCSPs

A PCSP is a combination of two CSPs defined by two similar templates; the computational question is to distinguish a YES instance of the first one from a NO instance of the second. The computational complexity of many PCSPs remains unknown. Even the case of Boolean templates (solved for CSP by Schaefer [STOC'78]) remains wide open. The main result of Brakensiek and Guruswami [SODA'18] shows that Boolean PCSPs exhibit a dichotomy (PTIME vs. NPC) when "all the clauses are symmetric and allow for negation of variables''. In this paper we remove the "allow for negation of variables'' assumption from the theorem. The "symmetric" assumption means that changing the order of variables in a constraint does not change its satisfiability. The "negation of variables" means that both of the templates share a relation which can be used to effectively negate Boolean variables. The main result of this paper establishes dichotomy for all the symmetric boolean templates. The tractability case of our theorem and the theorem of Brakensiek and Guruswami are almost identical. The main difference, and the main contribution of this work, is the new reason for hardness and the reasoning proving the split.

==> BasicRelaxations.tex <==
\section{Basic relaxations}\label{relax}

\begin{defn}
	Structure $\relstr A,\relstr B$ is a relaxation of a structure $\relstr A_0,\relstr B_0$ if and only if $\pol{\relstr A,\relstr B_0} \subseteq \pol \relstr A,\relstr B$.
\end{defn}

Those two facts follow from Galois correspondence \cite{PCSP17}:
\begin{itemize}
	\item If $\pol \relstr A,\relstr B \subseteq \pol{\relstr A,\relstr B '}$ then $\pcsp \relstr A,\relstr B \geq_\text{Log} \pcsp{\relstr A,\relstr B '}$
	\item If $\pol \relstr A,\relstr B = \pol{\relstr A,\relstr B '}$ then $\pcsp \relstr A,\relstr B \sim_\text{Log} \pcsp{\relstr A,\relstr B '}$
\end{itemize}

It's important to notice, that we can combine $\relstr A,\relstr B$ with it's relaxations without changing it's complexity. Also removing relations from structure can work as some relaxation, so it's easy to see that we can \textit{chaining} our relaxations.

\begin{relaxation}
	If structure $\relstr A,\relstr B$ is idempotent then both $\rel{0, 0,1}$ and $\rel{1, 1,1}$ are relaxations of $\relstr A,\relstr B$.
\end{relaxation}
\begin{proof}
	Assume otherwise, then there must be a function $f \in \pol \relstr A,\relstr B$ such that $f(\overline{0}) = 1$ or $f(\overline{1}) = 0$, which breaks assumption about idempotence -- contradiction.
\end{proof}

\begin{relaxation}
	If $\rel{I,J,n} \in \relstr A,\relstr B$ then $\rel{I,J,n}$ is a relaxation of $\relstr A,\relstr B$.
\end{relaxation}
\begin{proof}
	Every $f \in \pol \relstr A,\relstr B$ has to be compatible with every relation in $\relstr A,\relstr B$ so with $\rel{I,J,n}$ particularly.
\end{proof}

\begin{relaxation}
	If $\rel{I,J,n} \in \relstr A,\relstr B$ and $I' \subseteq I$, $J \subseteq J'$ then $\rel{I',J',n}$ is a relaxation of $\relstr A,\relstr B$.
\end{relaxation}
\begin{proof}
	Assume otherwise, then there must be a function $f \in \pol \relstr A,\relstr B$ and $\overline{x} \in I'$ such that $f(\overline{x}) \not \in J'$, but following is true:
	\[\overline{x} \in I' \implies \overline{x} \in I \implies f(\overline{x}) \in J  \implies f(\overline{x}) \in J '\]
	so contradiction.
\end{proof}

We will define two functions which will help us in showing next relaxations:

\begin{defn}
	\begin{align*}
		\LEFT{n}{I} &:= \{i-1: i \in I\} \cap \{0,\dotsc,n-1\}\\
		\RIGHT{n}{I} &:= I \cap \{0,\dotsc,n-1\}
	\end{align*}
\end{defn}

\begin{relaxation}[Moving left]
	If $R=\rel{I,J,n}, \textbf{1}=\rel{1, 1, 1} \in \relstr A,\relstr B$  then:
	\[S=\rel{\LEFT{n}{I},\LEFT{n}{J},n-1}\]
	 is a relaxation of $\relstr A,\relstr B$.
\end{relaxation}
\begin{proof}
	We will prove it by pp-defining $S$:
	\[S(\overline{x}) = \exists_y \textbf{1}(y) \land R(y, \overline{x})\]
\end{proof}

\begin{relaxation}[Moving right]
If $R=\rel{I,J,n}, \textbf{0}=\rel{0, 0, 1} \in \relstr A,\relstr B$  then:
 \[S=\rel{\RIGHT{n}{I},\RIGHT{n}{J},n-1}\] is a relaxation of $\relstr A,\relstr B$.
\end{relaxation}
\begin{proof}
We will prove it by pp-defining $S$:
\[S(\overline{x}) = \exists_y \textbf{0}(y) \land R(y, \overline{x})\]
\end{proof}

\begin{example}
	Let $\relstr A,\relstr B = (\rel{0, 0,1}, \rel{1, 1,1}, \printrel{0, 1, 4, 5}{0, \dotsc, 5}{5})$, then by applying \textit{"moving left"} relaxation once we will get relation $\printrel{0, 3, 4}{0, \dotsc, 4}{4})$ and then by applying \textit{"moving right"} relaxation on the result we will get $\printrel{0, 3}{0, \dotsc, 3}{3})$.
\end{example}


==> pcsptables.tex <==
\NeedsTeXFormat{LaTeX2e}
\usepackage[table,xcdraw]{xcolor}


\newcommand{\emptycolumns}[1]{\multicolumn{#1}{c}{}}

%#FFC53C
%#A58E65
%#FE8A7D
%#DFE0DF

\definecolor{orangex}{HTML}{FFC53C}
\definecolor{brownx}{HTML}{A58E65}
\definecolor{redx}{HTML}{FE8A7D}
\definecolor{grayx}{HTML}{DFE0DF}
\definecolor{whitexd}{HTML}{FFFFFF}



\newcommand{\unionofzerosetstable}{
	\begin{tabular}{llllllllllllll|l}
		\rowcolor{redx} 
		1                         & 1                         & 1                         & 1                         & 1                         & 1                         & 1                         & 1                         & 1                         & 0                     & 0                     & 0                     & 0                     & \cellcolor{brownx}0 & \cellcolor{orangex}1 \\
		\cellcolor{grayx}0 & 1                         & 1                         & 1                         & 1                         & 1                         & 1                         & 1                         & 1                         & 1                     & 1                     & 1                     & 1                     & \cellcolor{brownx}1 & \cellcolor{orangex}0 \\
		1                         & \cellcolor{grayx}0 & 1                         & 1                         & 1                         & 1                         & 1                         & 1                         & 1                         & \multicolumn{1}{r}{1} & \multicolumn{1}{r}{1} & \multicolumn{1}{r}{1} & \multicolumn{1}{r}{1} & \cellcolor{brownx}1 & \cellcolor{orangex}0 \\
		1                         & 1                         & \cellcolor{grayx}0 & 1                         & 1                         & 1                         & 1                         & 1                         & 1                         & \multicolumn{1}{r}{1} & \multicolumn{1}{r}{1} & \multicolumn{1}{r}{1} & \multicolumn{1}{r}{1} & \cellcolor{brownx}1 & \cellcolor{orangex}0 \\
		1                         & 1                         & 1                         & \cellcolor{grayx}0 & 1                         & 1                         & 1                         & 1                         & 1                         & \multicolumn{1}{r}{1} & \multicolumn{1}{r}{1} & \multicolumn{1}{r}{1} & \multicolumn{1}{r}{1} & \cellcolor{brownx}1 & \cellcolor{orangex}0 \\
		1                         & 1                         & 1                         & 1                         & \cellcolor{grayx}0 & 1                         & 1                         & 1                         & 1                         & 1                     & 1                     & 1                     & 1                     & \cellcolor{brownx}1 & \cellcolor{orangex}0 \\
		1                         & 1                         & 1                         & 1                         & 1                         & \cellcolor{grayx}0 & \cellcolor{grayx}0 & \cellcolor{grayx}0 & \cellcolor{grayx}0 & 1                     & 1                     & 1                     & 1                     & \cellcolor{brownx}1 & \cellcolor{orangex}0
	\end{tabular}
}

\newcommand{\flippingzerotable}{
	\begin{tabular}{lllllllllrrrrl
			|>{\columncolor{orangex}}l }
		\cellcolor{grayx}1 & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & \multicolumn{1}{l}{0}     & \multicolumn{1}{l}{0}     & \multicolumn{1}{l}{0}     & \multicolumn{1}{l}{0}     & 0                         & 1 \\
		0                         & \cellcolor{grayx}1 & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & \multicolumn{1}{l}{0}     & \multicolumn{1}{l}{0}     & \multicolumn{1}{l}{0}     & \multicolumn{1}{l}{0}     & 0                         & 1 \\
		0                         & 0                         & \cellcolor{grayx}1 & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 1 \\
		0                         & 0                         & 0                         & \cellcolor{redx}1 & \cellcolor{redx}1 & \cellcolor{redx}1 & \cellcolor{redx}1 & \cellcolor{redx}1 & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 1 \\
		0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & \cellcolor{grayx}1 & \cellcolor{grayx}1 & \cellcolor{grayx}1 & \cellcolor{grayx}1 & \cellcolor{grayx}1 & \cellcolor{grayx}1 & 1\\
		\hline
	\end{tabular}
	\begin{tabular}{lllllllllrrrrl
			|>{\columncolor{orangex}}l }
		\cellcolor{grayx}1 & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & \multicolumn{1}{l}{0}     & \multicolumn{1}{l}{0}     & \multicolumn{1}{l}{0}     & \multicolumn{1}{l}{0}     & 0                         & 1 \\
		0                         & \cellcolor{grayx}1 & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & \multicolumn{1}{l}{0}     & \multicolumn{1}{l}{0}     & \multicolumn{1}{l}{0}     & \multicolumn{1}{l}{0}     & 0                         & 1 \\
		0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0 \\
		0                         & 0                         & \cellcolor{brownx}1 & \cellcolor{redx}1 & \cellcolor{redx}1 & \cellcolor{redx}1 & \cellcolor{redx}1 & \cellcolor{redx}1 & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0 \\
		0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & \cellcolor{grayx}1 & \cellcolor{grayx}1 & \cellcolor{grayx}1 & \cellcolor{grayx}1 & \cellcolor{grayx}1 & \cellcolor{grayx}1 & 1
	\end{tabular}
}
\newcommand{\flippingonetable}{
	\begin{tabular}{lllllllllrrrrl
			|>{\columncolor{orangex}}l }
		\cellcolor{grayx}1 & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & \multicolumn{1}{l}{0}     & \multicolumn{1}{l}{0}     & \multicolumn{1}{l}{0}     & \multicolumn{1}{l}{0}     & 0                         & 1 \\
		0                         & \cellcolor{grayx}1 & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & \multicolumn{1}{l}{0}     & \multicolumn{1}{l}{0}     & \multicolumn{1}{l}{0}     & \multicolumn{1}{l}{0}     & 0                         & 1 \\
		0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0 \\
		0                         & 0                         & \cellcolor{redx}1             & \cellcolor{redx}1 & \cellcolor{redx}1 & \cellcolor{redx}1 & \cellcolor{redx}1 & \cellcolor{redx}1 & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 1 \\
		0                         & 0                         & 0 & 0                         & 0                         & 0                         & 0                         & 0                         & \cellcolor{grayx}1 & \cellcolor{grayx}1 & \cellcolor{grayx}1 & \cellcolor{grayx}1 & \cellcolor{grayx}1 & \cellcolor{grayx}1 & 0 \\
		\hline
	\end{tabular}
	
	\begin{tabular}{lllllllllrrrrl
			|>{\columncolor{orangex}}l }
		\cellcolor{grayx}1 & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & \multicolumn{1}{l}{0}     & \multicolumn{1}{l}{0}     & \multicolumn{1}{l}{0}     & \multicolumn{1}{l}{0}     & 0                         & 1 \\
		0                         & \cellcolor{grayx}1 & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & \multicolumn{1}{l}{0}     & \multicolumn{1}{l}{0}     & \multicolumn{1}{l}{0}     & \multicolumn{1}{l}{0}     & 0                         & 1 \\
		0                         & 0                         & \cellcolor{brownx}1                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 1 \\
		0                         & 0                         & 0             & \cellcolor{redx}1 & \cellcolor{redx}1 & \cellcolor{redx}1 & \cellcolor{redx}1 & \cellcolor{redx}1 & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0 \\
		0                         & 0                         & 0 & 0                         & 0                         & 0                         & 0                         & 0                         & \cellcolor{grayx}1 & \cellcolor{grayx}1 & \cellcolor{grayx}1 & \cellcolor{grayx}1 & \cellcolor{grayx}1 & \cellcolor{grayx}1 & 0 \\
	\end{tabular}
}

\newcommand{\tablexd}{
		\begin{tabular}{
				lllllllllllllllll
				|>{\columncolor{orangex}}l }
				\cellcolor{grayx}1 & \cellcolor{grayx}1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 \\
				0 & 0 & \cellcolor{grayx}1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 \\
				0 & 0 & 0 & \cellcolor{grayx}1 & \cellcolor{grayx}1 & \cellcolor{grayx}1 & \cellcolor{grayx}1 & \cellcolor{grayx}1 & \cellcolor{grayx}1 & \multicolumn{1}{r}{\cellcolor{whitexd}0} & \multicolumn{1}{r}{\cellcolor{whitexd}0} & \multicolumn{1}{r}{\cellcolor{whitexd}0} & \multicolumn{1}{r}{\cellcolor{whitexd}0} & 0 & 0 & 0 & 0 & 1 \\
				\cellcolor{redx}0 & \cellcolor{redx}0 & \cellcolor{redx}0 & \cellcolor{redx}0 & \cellcolor{redx}0 & \cellcolor{redx}0 & \cellcolor{redx}0 & \cellcolor{redx}0 & \cellcolor{redx}0 & \multicolumn{1}{r}{\cellcolor{whitexd}1} & \multicolumn{1}{r}{\cellcolor{whitexd}1} & \multicolumn{1}{r}{\cellcolor{whitexd}1} & \multicolumn{1}{r}{\cellcolor{whitexd}1} & 1 & 1 & 1 & 1 & 0 \\
		\end{tabular}
}

\newcommand{\tablexda}{

\begin{tabular}{lllllllllrrrrllllllll
		|>{\columncolor{orangex}}l }
	
	\cellcolor{grayx}0 & \cellcolor{grayx}0 & \cellcolor{grayx}0 & 1                         & 1                         & 1                         & 1                         & 1                         & 1                         & \multicolumn{1}{l}{1}     & \multicolumn{1}{l}{1}     & \multicolumn{1}{l}{1}     & \multicolumn{1}{l}{1}     & 1                         & 1                         & 1                         & 1                         & 1                         & 1                         & 1                         & 1                                                  & 0 \\
	1                         & 1                         & 1                         & \cellcolor{grayx}0 & \cellcolor{grayx}0 & \cellcolor{grayx}0 & 1                         & 1                         & 1                         & \multicolumn{1}{l}{1}     & \multicolumn{1}{l}{1}     & \multicolumn{1}{l}{1}     & \multicolumn{1}{l}{1}     & 1                         & 1                         & 1                         & 1                         & 1                         & 1                         & 1                         & 1                                                  & 0 \\
	1                         & 1                         & 1                         & 1                         & 1                         & 1                         & \cellcolor{grayx}0 & \cellcolor{grayx}0 & \cellcolor{grayx}0 & 1                         & 1                         & 1                         & 1                         & 1                         & 1                         & 1                         & 1                         & 1                         & 1                         & 1                         & 1                                                  & 0 \\
	1                         & 1                         & 1                         & 1                         & 1                         & 1                         & 1                         & 1                         & 1                         & \cellcolor{redx}0 & \cellcolor{redx}0 & \cellcolor{redx}0 & \cellcolor{redx}0 & \cellcolor{redx}0 & \cellcolor{redx}0 & 1                         & 1                         & \cellcolor{brownx}1                         & 1                         & 1                         & 1                                                 & 0 \\
	\cellcolor{grayx}1                         & \cellcolor{grayx}1                         & \cellcolor{grayx}1                         & \cellcolor{grayx}1                         & \cellcolor{grayx}1                         & \cellcolor{grayx}1                         & \cellcolor{grayx}1                         & \cellcolor{grayx}1                         & \cellcolor{grayx}1                         & \cellcolor{grayx}1                         & \cellcolor{grayx}1                         & \cellcolor{grayx}1                         & \cellcolor{grayx}1                         & \cellcolor{grayx}1                         & \cellcolor{grayx}1                         & 0 & 0 & \cellcolor{brownx}0 & 0 & 0 & 0 & 1\\
	\hline
\end{tabular}

\begin{tabular}{lllllllllrrrrllllllll
		|>{\columncolor{orangex}}l }
	
	\cellcolor{grayx}0 & \cellcolor{grayx}0 & \cellcolor{grayx}0 & 1                         & 1                         & 1                         & 1                         & 1                         & 1                         & \multicolumn{1}{l}{1}     & \multicolumn{1}{l}{1}     & \multicolumn{1}{l}{1}     & \multicolumn{1}{l}{1}     & 1                         & 1                         & 1                         & 1                         & 1                         & 1                         & 1                         & 1                                                  & 0 \\
	1                         & 1                         & 1                         & \cellcolor{grayx}0 & \cellcolor{grayx}0 & \cellcolor{grayx}0 & 1                         & 1                         & 1                         & \multicolumn{1}{l}{1}     & \multicolumn{1}{l}{1}     & \multicolumn{1}{l}{1}     & \multicolumn{1}{l}{1}     & 1                         & 1                         & 1                         & 1                         & 1                         & 1                         & 1                         & 1                                                  & 0 \\
	1                         & 1                         & 1                         & 1                         & 1                         & 1                         & \cellcolor{grayx}0 & \cellcolor{grayx}0 & \cellcolor{grayx}0 & 1                         & 1                         & 1                         & 1                         & 1                         & 1                         & 1                         & 1                         & 1                         & 1                         & 1                         & 1                                                  & 0 \\
	1                         & 1                         & 1                         & 1                         & 1                         & 1                         & 1                         & 1                         & 1                         & \cellcolor{redx}0 & \cellcolor{redx}0 & \cellcolor{redx}0 & \cellcolor{redx}0 & \cellcolor{redx}0 & \cellcolor{redx}0 & 1                         & 1                         & \cellcolor{brownx}0                         & 1                         & 1                         & 1                                                 & 1 \\
	\cellcolor{grayx}1                         & \cellcolor{grayx}1                         & \cellcolor{grayx}1                         & \cellcolor{grayx}1                         & \cellcolor{grayx}1                         & \cellcolor{grayx}1                         & \cellcolor{grayx}1                         & \cellcolor{grayx}1                         & \cellcolor{grayx}1                         & \cellcolor{grayx}1                         & \cellcolor{grayx}1                         & \cellcolor{grayx}1                         & \cellcolor{grayx}1                         & \cellcolor{grayx}1                         & \cellcolor{grayx}1                         & 0 & 0 & \cellcolor{brownx}1 & 0 & 0 & 0 & 0\\
\end{tabular}
}


\newcommand{\anisat}{
\begin{tabular}{lllllllll | l}
	\rowcolor{grayx}
	1                         & 1                         & 1                         & 1                         & 1                         & 1                         & 1                         & 1                         & \cellcolor{redx}1 & \cellcolor{orangex}1 \\
	\rowcolor{grayx}
	1                         & 1                         & 1                         & 1                         & 1                         & 1                         & 1                         & 1                         & \cellcolor{redx}1 & \cellcolor{orangex}1 \\
	\cellcolor{brownx}1 & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & \cellcolor{redx}0 & \cellcolor{orangex}1 \\
	0                         & \cellcolor{brownx}1 & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & \cellcolor{redx}0 & \cellcolor{orangex}1 \\
	0                         & 0                         & \cellcolor{brownx}1 & 0                         & 0                         & 0                         & 0                         & 0                         & \cellcolor{redx}0 & \cellcolor{orangex}1 \\
	0                         & 0                         & 0                         & \cellcolor{brownx}1 & 0                         & 0                         & 0                         & 0                         & \cellcolor{redx}0 & \cellcolor{orangex}1 \\
	0                         & 0                         & 0                         & 0                         & \cellcolor{brownx}1 & \cellcolor{brownx}1 & \cellcolor{brownx}1 & \cellcolor{brownx}1 & \cellcolor{redx}1 & \cellcolor{orangex}0 \\
	\rowcolor{grayx}
	0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & \cellcolor{redx}0 & \cellcolor{orangex}0 \\
	\rowcolor{grayx}
	0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & \cellcolor{redx}0 & \cellcolor{orangex}0
\end{tabular}

}

\newcommand{\anisatxd}{
\begin{tabular}{
		>{\columncolor{brownx}}l
		>{\columncolor{brownx}}l
		>{\columncolor{brownx}}l
		>{\columncolor{brownx}}l
		>{\columncolor{redx}}l
		|>{\columncolor{orangex}}l }
	0                  & 1                  & 1                  & 0                  & 0 & 1 \\
	0                  & 0                  & 1                  & 1                  & 0 & 1 \\
	1                  & 0                  & 0                  & 1                  & 0 & 1 \\
	1                  & 1                  & 0                  & 0                  & 0 & 1 \\
	\cellcolor{grayx}1 & \cellcolor{grayx}1 & \cellcolor{grayx}1 & \cellcolor{grayx}1 & 1 & 1 \\
	\cellcolor{grayx}1 & \cellcolor{grayx}1 & \cellcolor{grayx}1 & \cellcolor{grayx}1 & 1 & 1
\end{tabular}

}


\newcommand{\noextremesflipone}{
\begin{tabular}{llllllllllllll|
			>{\columncolor{orangex}}l }
		\cellcolor{grayx}1 & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0 & 0 & 0                     & 0                     & 0                     & 0                     & 0 & 1 \\
		\cellcolor{grayx}1 & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0 & 0 & 0                     & 0                     & 0                     & 0                     & 0 & 1 \\
		\cellcolor{grayx}1 & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0 & 0 & \multicolumn{1}{r}{0} & \multicolumn{1}{r}{0} & \multicolumn{1}{r}{0} & \multicolumn{1}{r}{0} & 0 & 1 \\
		0                         & \cellcolor{grayx}1 & 0                         & 0                         & 0                         & 0                         & 0                         & 0 & 0 & \multicolumn{1}{r}{0} & \multicolumn{1}{r}{0} & \multicolumn{1}{r}{0} & \multicolumn{1}{r}{0} & 0 & 1 \\
		0                         & \cellcolor{redx}1 & \cellcolor{redx}1 & \cellcolor{redx}1 & \cellcolor{redx}1 & \cellcolor{redx}1 & \cellcolor{redx}1 & 0 & 0 & 0                     & 0                     & 0                     & 0                     & 0 & 1 \\
		0                         & \cellcolor{redx}1 & \cellcolor{redx}1 & \cellcolor{redx}1 & \cellcolor{redx}1 & \cellcolor{redx}1 & \cellcolor{redx}1 & 0 & 0 & 0                     & 0                     & 0                     & 0                     & 0 & 1 \\
		0                         & \cellcolor{brownx}0 & \cellcolor{redx}1 & \cellcolor{redx}1 & \cellcolor{redx}1 & \cellcolor{redx}1 & \cellcolor{redx}1 & 0 & 0 & 0                     & 0                     & 0                     & 0                     & 0 & 0
\end{tabular}
}

\newcommand{\noextremesflipzero}{
	\begin{tabular}{llllllllllllll|
			>{\columncolor{orangex}}l }
		\cellcolor{grayx}1 & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0 & 0 & 0                     & 0                     & 0                     & 0 & 1 \\
		\cellcolor{grayx}1 & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0 & 0 & 0                     & 0                     & 0                     & 0 & 1 \\
		\cellcolor{grayx}1 & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0 & 0 & \multicolumn{1}{r}{0} & \multicolumn{1}{r}{0} & \multicolumn{1}{r}{0} & 0 & 1 \\
		0                         & \cellcolor{grayx}1 & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0 & 0 & \multicolumn{1}{r}{0} & \multicolumn{1}{r}{0} & \multicolumn{1}{r}{0} & 0 & 1 \\
		0                         & \cellcolor{brownx}1 & \cellcolor{redx}1 & \cellcolor{redx}1 & \cellcolor{redx}1 & \cellcolor{redx}1 & \cellcolor{redx}1 & \cellcolor{redx}1 & 0 & 0 & 0                     & 0                     & 0                     & 0 & 0 \\
		0                         & \cellcolor{brownx}1 & \cellcolor{redx}1 & \cellcolor{redx}1 & \cellcolor{redx}1 & \cellcolor{redx}1 & \cellcolor{redx}1 & \cellcolor{redx}1 & 0 & 0 & 0                     & 0                     & 0                     & 0 & 0 \\
		0                         & 0                         & \cellcolor{redx}1 & \cellcolor{redx}1 & \cellcolor{redx}1 & \cellcolor{redx}1 & \cellcolor{redx}1 & \cellcolor{redx}1 & 0 & 0 & 0                     & 0                     & 0                     & 0 & 1
	\end{tabular}
}

\newcommand{\creatingonesets}{
\begin{tabular}{lllllllllll | l}
	\cellcolor{orangex}0 & \cellcolor{redx}1 & \cellcolor{redx}1 & \cellcolor{redx}1 & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & \cellcolor{orangex}0   \\
	\cellcolor{redx}1 & \cellcolor{redx}1 & \cellcolor{orangex}0 & \cellcolor{redx}1 & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & 0                         & \cellcolor{orangex}{\color[HTML]{000000} 0}   \\
	\rowcolor{grayx}
	1                         & 0                         & 1                         & 0                         & 0                         & 0                         & 0                         & 0                         & 1                         & 0                         & 1                         & \cellcolor{orangex}{\color[HTML]{000000} 0/1} \\
	0                         & 0                         & 0                         & 0                         & \cellcolor{brownx}1 & \cellcolor{brownx}1 & \cellcolor{brownx}1 & \cellcolor{brownx}1 & \cellcolor{brownx}0 & \cellcolor{brownx}1 & \cellcolor{brownx}1 & \cellcolor{orangex}{\color[HTML]{000000} 0}   \\
	0                         & 0                         & 0                         & 0                         & \cellcolor{brownx}1 & \cellcolor{brownx}1 & \cellcolor{brownx}1 & \cellcolor{brownx}1 & \cellcolor{brownx}1 & \cellcolor{brownx}1 & \cellcolor{brownx}0 & \cellcolor{orangex}{\color[HTML]{000000} 0}
\end{tabular}
}

\newcommand{\lasttable}{
\begin{tabular}{
		>{\columncolor{grayx}}l 
		>{\columncolor{grayx}}l 
		>{\columncolor{grayx}}l 
		>{\columncolor{grayx}}l clllclllclll}
	\hline
	\cline{5-8}
	\multicolumn{4}{|c}{\cellcolor{grayx}}                           & \cellcolor{orangex}1 & \cellcolor{orangex}1 & \cellcolor{orangex}... & \cellcolor{orangex}1 & \multicolumn{4}{c}{\cellcolor{brownx}}                           & \multicolumn{4}{c|}{}                           \\ 

	\multicolumn{4}{|c}{\cellcolor{grayx}}                           & \multicolumn{4}{c}{}                                                                                                                                                        & \multicolumn{4}{c}{\cellcolor{brownx}}                           & \multicolumn{4}{c|}{}                           \\
	\multicolumn{4}{|c}{\cellcolor{grayx}}                           & \multicolumn{4}{c}{}                                                                                                                                                        & \multicolumn{4}{c}{\cellcolor{brownx}\ \ \ \ \ \ \ \ \ \ \ \ \ \ }                           & \multicolumn{4}{c|}{}                           \\
	\multicolumn{4}{|c}{\multirow{-4}{*}{\cellcolor{grayx}\Huge$1$}} & \multicolumn{4}{c}{\multirow{-3}{*}{\huge$0$}}                                                                                                                              & \multicolumn{4}{c}{\multirow{-4}{*}{\cellcolor{brownx}\Huge$I_m$}} & \multicolumn{4}{c|}{\multirow{-4}{*}{\Huge$0$}} \\
	\multicolumn{4}{|l}{\cellcolor{grayx}}                           & \multicolumn{12}{c|}{\cellcolor{redx}}                                                                                                                                                                                                                                                                                                         \\
	\multicolumn{4}{|l}{\cellcolor{grayx}}                           & \multicolumn{12}{c|}{\cellcolor{redx}}                                                                                                                                                                                                                                                                                                         \\
	\multicolumn{4}{|l}{\cellcolor{grayx}}                           & \multicolumn{12}{c|}{\cellcolor{redx}}                                                                                                                                                                                                                                                                                                         \\
	\multicolumn{4}{|l}{\multirow{-4}{*}{\cellcolor{grayx}\Huge$0$}} & \multicolumn{12}{c|}{\multirow{-4}{*}{\cellcolor{redx}\Huge$E''$}}\\
	\hline                                                                                                                                                                                                                                                                            
\end{tabular}

}





\newcommand{\gaptable}{
\begin{tabular}{llllllllll
		|>{\columncolor{orangex}}l }
	\cellcolor{redx}1 & 0                         & 0                         & 0                         & 0                         & \cellcolor{redx}{\color[HTML]{000000} 1} & \cellcolor{redx}{\color[HTML]{000000} 1} & \cellcolor{redx}{\color[HTML]{000000} 1} & \cellcolor{redx}{\color[HTML]{000000} 1} & \cellcolor{redx}{\color[HTML]{000000} 1} & 1 \\
	0                         & \cellcolor{redx}1 & 0                         & 0                         & 0                         & \cellcolor{redx}1                        & \cellcolor{redx}1                        & \cellcolor{redx}1                        & \cellcolor{redx}1                        & \cellcolor{redx}1                        & 1 \\
	0                         & 0                         & \cellcolor{redx}1 & 0                         & 0                         & \cellcolor{redx}1                        & \cellcolor{redx}1                        & \cellcolor{redx}1                        & \cellcolor{redx}1                        & \cellcolor{redx}1                        & 1 \\
	0                         & 0                         & 0                         & \cellcolor{redx}1 & \cellcolor{redx}1 & \cellcolor{redx}1                        & \cellcolor{redx}1                        & \cellcolor{redx}1                        & \cellcolor{redx}1                        & \cellcolor{redx}1                        & 1 \\
	\cellcolor{grayx}0 & \cellcolor{grayx}0 & \cellcolor{grayx}0 & \cellcolor{grayx}0 & \cellcolor{grayx}0 & 1                                                & 1                                                & 1                                                & 1                                                & 1                                                & 0 \\
	\cellcolor{grayx}0 & \cellcolor{grayx}0 & \cellcolor{grayx}0 & \cellcolor{grayx}0 & \cellcolor{grayx}0 & 1                                                & 1                                                & 1                                                & 1                                                & 1                                                & 0 \\
	\cellcolor{grayx}0 & \cellcolor{grayx}0 & \cellcolor{grayx}0 & \cellcolor{grayx}0 & \cellcolor{grayx}0 & 1                                                & 1                                                & 1                                                & 1                                                & 1                                                & 0
\end{tabular}}


\newcommand{\starexample}{
	\begin{tabular}{llllllllll
			|>{\columncolor{orangex}}l }
		0                         & 0                         & 0                         & \cellcolor{redx}1 & 0                         & 0                         & \cellcolor{redx}1 & 0                         & 0                         & 0                         & 1 \\
		\cellcolor{redx}1 & \cellcolor{redx}1 & \cellcolor{redx}1 & \cellcolor{redx}1 & \cellcolor{redx}1 & \cellcolor{redx}1 & 0                         & 0                         & 0                         & 0                         & 1 \\
		0                         & 0                         & 0                         & 0                         & \cellcolor{redx}1 & \cellcolor{redx}1 & \cellcolor{redx}1 & \cellcolor{redx}1 & \cellcolor{redx}1 & \cellcolor{redx}1 & 1 \\
		\cellcolor{redx}1 & \cellcolor{redx}1 & \cellcolor{redx}1 & 0                         & 0                         & 0                         & 0                         & \cellcolor{redx}1 & \cellcolor{redx}1 & \cellcolor{redx}1 & 1
	\end{tabular}}
